Stalnaker's Epistemic Logic in Isabelle/HOL

The foundations of formal models for epistemic and doxastic logics often rely on certain logical aspects of modal logics such as S4 and S4.2 and their semantics; however, the corresponding mathematical results are often stated in papers or books without including a detailed proof, or a reference to it, that allows the reader to convince themselves about them. We reinforce the foundations of the epistemic logic S4.2 for countably many agents by formalizing its soundness and completeness results for the class of all weakly-directed pre-orders in the proof assistant Isabelle/HOL. This logic corresponds to the knowledge fragment, i.e., the logic for formulas that may only include knowledge modalities in Stalnaker's system for knowledge and belief. Additionally, we formalize the equivalence between two axiomatizations for S4, which are used depending on the type of semantics given to the modal operators, as one is commonly used for the relational semantics, and the other one arises naturally from the topological semantics.

==> eptcsdata.tex <==
\providecommand{\firstpage}{4}
\providecommand{\publicationstatus}{Temur Kutsia, Daniel Ventura, David Monniaux \&\\
 Jos\'e F. Morales (Eds.): LSFA 2023 + HCVS 2023\\
EPTCS 402, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.402.4}{10.4204/EPTCS.402.4}}
\pdfoutput=1

